State World Models: Execute the Rules, Generate the Pixels

Existing world models can generate action-conditioned video from a single image. Many focus on camera movement, allowing users to explore the generated scene. However, navigation alone does not ensure that an action follows persistent rules when its outcome depends on state that is invisible in the current frame. We present Stateful Harness, a framework that separates world evolution from video rendering to support stateful and rule-governed interaction. It maintains an evolving world state under specified rules, renders each resulting event with a frozen video model, and uses the generated clip to update the world state for the next turn. At each turn, the harness resolves the action selected by the user and compiles the resulting event into an instruction, while a preview clip from an editable 3D scene provides spatial and camera guidance. To evaluate rule compliance, we build WorldState-Bench, a benchmark of 50 counterfactual twin pairs that share an initial frame and action but differ in hidden state and required outcome. Under rule-only prompting, the best of the 11 evaluated video backends produces the required endings for both cases in 32% of pairs. For MiniMax-H3, specifying the required endings raises this rate from 32% to 64%, while the full harness reaches 92% with the same frozen model. These results support separating rule execution from video rendering for world interactions with hidden state.

==> figures/fig_framework.tex <==
% ------------------------------------------------------------------
% Figure: The Stateful Harness, staged.
%   (a) Stage 1 -- setup (once per world, per twin)
%   (b) Stage 2 -- turn loop (every turn, with user interaction)
% The clay model is drawn as what it is: a floor plane plus a few
% untextured cuboids. Dashed slots reserve positions for intermediate
% artifacts; they can be replaced by real renders via \includegraphics.
% Absolute-coordinate layout (canvas ~190 x 140mm); \resizebox scales
% to 0.9\textwidth.
% ------------------------------------------------------------------
\begin{figure}[t]
\centering
\resizebox{0.7\textwidth}{!}{%
\begin{tikzpicture}[
  font=\scriptsize, x=1mm, y=1mm,
  arr/.style={-{Latex[length=2mm]}, line width=0.8pt, black!70},
  channel/.style={-{Latex[length=2.2mm]}, line width=1.0pt},
  flow/.style={-{Latex[length=1.8mm]}, line width=0.6pt, black!70},
  feedback/.style={-{Latex[length=1.8mm]}, line width=0.6pt, black!55, dashed},
  srcbox/.style={draw=black!55, rounded corners=1.5pt, thick, fill=inputlav!50, align=center, inner sep=2pt},
  procbox/.style={draw=black!55, rounded corners=1.5pt, thick, fill=white, align=center, inner sep=2pt},
  devrow/.style={draw=black!55, rounded corners=1.5pt, thick, align=center, inner sep=2.2pt},
  lane/.style={font=\tiny\bfseries, black!55, rotate=90},
  note/.style={font=\tiny, black!60, align=left},
  slot/.style={densely dashed, rounded corners=1.5pt, fill=white, line width=0.55},
]

% ---------- placeholder glyphs ----------
\newcommand{\imgglyph}[2]{%
  \begin{scope}[shift={(#1,#2)}]
    \draw[black!40, rounded corners=0.6pt, line width=0.4] (-3.2,-1.9) rectangle (3.2,1.9);
    \fill[black!30] (-2.2,-0.9) -- (-0.7,1.0) -- (0.6,-0.9) -- cycle;
    \fill[black!30] (0.2,-0.9) -- (1.3,0.3) -- (2.3,-0.9) -- cycle;
    \fill[black!30] (1.7,1.0) circle (0.4);
  \end{scope}}
\newcommand{\docglyph}[2]{%
  \begin{scope}[shift={(#1,#2)}]
    \draw[black!40, rounded corners=0.6pt, line width=0.4] (-2.8,-1.9) rectangle (2.8,1.9);
    \draw[black!40, line width=0.35] (-1.8,1.1) -- (1.8,1.1);
    \draw[black!40, line width=0.35] (-1.8,0.3) -- (1.8,0.3);
    \draw[black!40, line width=0.35] (-1.8,-0.5) -- (1.0,-0.5);
    \draw[black!40, line width=0.35] (-1.8,-1.3) -- (1.4,-1.3);
  \end{scope}}

% ---------- clay-model glyph: floor plane + a few cuboids ----------
% #1,#2 = lower-left of the bounding area; scene drawn ~16 wide, 10 tall
\newcommand{\wbox}[4]{% x,y (front-bottom-left), width, height
  \draw[black!50, fill=white, line width=0.45] (#1,#2) rectangle ({#1+#3},{#2+#4});
  \draw[black!50, fill=black!6, line width=0.45]
    ({#1},{#2+#4}) -- ({#1+1.3},{#2+#4+0.8}) -- ({#1+#3+1.3},{#2+#4+0.8})
    -- ({#1+#3},{#2+#4}) -- cycle;
  \draw[black!50, fill=black!14, line width=0.45]
    ({#1+#3},{#2}) -- ({#1+#3+1.3},{#2+0.8}) -- ({#1+#3+1.3},{#2+#4+0.8})
    -- ({#1+#3},{#2+#4}) -- cycle;}
\newcommand{\whitescene}[2]{%
  \begin{scope}[shift={(#1,#2)}]
    \draw[black!35, fill=black!4, line width=0.4]
      (-8,-3.4) -- (8,-3.4) -- (10.4,-5.2) -- (-5.6,-5.2) -- cycle;
    \wbox{-6.2}{-3.4}{3.4}{4.2}
    \wbox{-1.2}{-3.4}{2.2}{2.2}
    \wbox{2.6}{-3.4}{4.6}{3.0}
  \end{scope}}

% ================= (a) Stage 1: setup =================
\draw[black!55, rounded corners=3pt, thick, fill=black!3] (2,90) rectangle (188,138);
\node[font=\small\bfseries, anchor=north] at (95,137.2)
  {(a) Stage 1: setup {\normalfont\scriptsize\itshape --- once per world, per twin}};

% lane 1: rules
\node[lane] at (6,124) {rules};
\node[srcbox, minimum width=34mm, minimum height=11mm] at (28,124) {\textbf{Game story}\\\& design doc};
\draw[arr] (45.5,124) -- (50,124);
\node[procbox, minimum width=54mm, minimum height=11mm] at (78.5,124)
  {Rule-program agent: write $\tau$ in the rule\\ language, validate, freeze (shared by twins)};
\draw[arr] (106,124) -- (111,124);
\draw[slot, draw=black!50, fill=black!4] (112,117.5) rectangle (132,130.5);
\docglyph{122}{125.4};
\node[font=\tiny, black!60] at (122,119.6) {rule program};
% (note removed: inset claims this corner)

% lane 2: frame
\node[lane] at (6,110) {frame};
\node[srcbox, minimum width=34mm, minimum height=11mm] at (28,110) {\textbf{User's image}\\(any photo / screenshot)};
\draw[arr] (45.5,110) -- (50,110);
\node[procbox, minimum width=54mm, minimum height=11mm] at (78.5,110)
  {Frame intake: geometry lift seeds the white\\model from the supplied first frame};
\draw[arr] (106,110) -- (111,110);
\draw[slot, draw=black!50, fill=black!4] (112,103.5) rectangle (132,116.5);
\node[font=\tiny\itshape, text=black!45, align=center] at (122,110)
  {first frame $I_0$\\[1pt]{\tiny photo slot}};
\node[note, anchor=west] at (136,110) {pixels shared\\by the twins};

% lane 3: state
\node[lane] at (6,96) {state};
\node[srcbox, minimum width=34mm, minimum height=11mm] at (28,96) {\textbf{Twin spec:} theme,\\twin id, seeds};
\draw[arr] (45.5,96) -- (50,96);
\node[procbox, minimum width=54mm, minimum height=11mm] at (78.5,96)
  {Ledger + scene init: hidden variables\\$z_A \neq z_B$, initial clay-model layout $u_0$};
\draw[arr] (106,96) -- (111,96);
\draw[slot, draw=black!50, fill=black!4] (112,89.5) rectangle (132,102.5);
\docglyph{118}{98.6};
\node[font=\tiny, black!60] at (122,91.4) {ledger $z_A / z_B$};
\draw[slot, draw=spatialorangedark, fill=spatialorange!10] (136,89.5) rectangle (156,102.5);
\begin{scope}[shift={(146,96.2)}, scale=0.62]\whitescene{0}{0}\end{scope}
\node[font=\tiny, text=spatialorangedark] at (146,91.4) {clay model $u_0$};

% ---------- game-definition inset: the four primitives ----------
% and the transition relation the notebook specifies:
% rules read (state, action) and write the next state; goals end the episode.
\draw[black!55, rounded corners=2pt, thick, fill=white] (157,91.5) rectangle (186,131);
\node[font=\tiny\bfseries, black!70] at (171.5,128.8) {game definition};
\node[devrow, font=\tiny, fill=inputlav!50, minimum width=13mm, minimum height=6mm]
  at (163.8,121) (ga) {\textbf{Action} $a_t$};
\node[devrow, font=\tiny, fill=harnessblue!35, minimum width=13mm, minimum height=7.5mm]
  at (179.2,121) (gs) {\textbf{State} $S_t$\\[-2pt]{\tiny text $\cdot$ spatial}};
\node[devrow, font=\tiny, fill=white, minimum width=13mm, minimum height=6mm]
  at (171.5,106.5) (gr) {\textbf{Rules} $\tau$};
\node[devrow, font=\tiny, fill=contgreen!50, minimum width=11.5mm, minimum height=5.5mm]
  at (163.8,94.5) (gg) {\textbf{Goals}};
\node[devrow, font=\tiny, fill=white, minimum width=13mm, minimum height=5.5mm]
  at (179,94.5) (gs2) {\textbf{State} $S_{t+1}$};
\draw[flow] (ga.south) -- (gr.150) node[pos=0.45, left=0.5mm, font=\tiny, black!60]{issue};
\draw[flow] (gs.south) -- (gr.30) node[pos=0.45, right=0.5mm, font=\tiny, black!60]{read};
\draw[flow] (gr.south) -- (gs2.north) node[pos=0.5, right=0.5mm, font=\tiny, black!60]{write};
\draw[feedback] (gg.north) -- (gr.220) node[pos=0.5, left=0.5mm, font=\tiny, black!55]{end?};

% ---------- transition ----------
\draw[arr, line width=1.2pt] (95,89.5) -- (95,79.2);
\node[font=\tiny, black!60, anchor=west, align=left] at (98,84.3)
  {artifacts loaded: frozen rules $\cdot$ first frame $I_0$ $\cdot$ initial ledger $z_0$ $\cdot$ initial scene $u_0$};

% ================= (b) Stage 2: turn loop =================
\draw[harnessbluedark, rounded corners=3pt, very thick, fill=harnessblue!8] (2,13) rectangle (188,78);
\node[font=\small\bfseries, text=harnessbluedark, anchor=north] at (95,77.2)
  {(b) Stage 2: turn loop {\normalfont\scriptsize\itshape --- every turn, driven by the user}};

% user + interaction input
\draw[black!55, rounded corners=2.5pt, thick, fill=inputlav!35] (4,26) rectangle (30,70);
\node[font=\tiny\bfseries, black!70] at (17,67.4) {User};
% stick figure
\begin{scope}[shift={(17,57)}]
  \draw[black!60, line width=0.6] (0,3.1) circle (1.15);
  \draw[black!60, line width=0.6] (0,1.95) -- (0,-1.2);
  \draw[black!60, line width=0.6] (-1.7,0.9) -- (1.7,0.9);
  \draw[black!60, line width=0.6] (0,-1.2) -- (-1.2,-3.1);
  \draw[black!60, line width=0.6] (0,-1.2) -- (1.2,-3.1);
\end{scope}
\node[draw=black!50, rounded corners=1.2pt, fill=white, line width=0.5,
      align=center, inner sep=1.6pt, font=\tiny] at (17,45.5)
  {move: WASD / arrows / camera\\[1pt]
   \emph{or} text action\\[1pt] ``open the chest''};
\node[srcbox, minimum width=20mm, minimum height=7mm] at (17,33.5) {\textbf{action} $a_t$};
\draw[arr] (30,47) -- (34.5,47);

% harness container
\draw[harnessbluedark, rounded corners=2.5pt, thick, fill=white] (35,22) rectangle (94,72);
\node[devrow, anchor=north, minimum width=54mm, fill=harnessblue!22] at (64.5,70.5) (r1)
  {\textbf{1. Settle}: rule engine $\tau$ + hidden-state ledger $S_{\mathrm{sem}}$\\
   {\tiny what happens --- twin identity decides}};
\node[devrow, anchor=north, minimum width=54mm, fill=spatialorange!60] at (64.5,60.5) (r2)
  {\textbf{2.} \textbf{White-model update}: edit instructions\\
   {\tiny where --- scene change / move / destroy}};
\node[devrow, anchor=north, minimum width=54mm, fill=harnessblue!60] at (64.5,50.5) (r3)
  {\textbf{3.} \textbf{\vsm{} compiler}: native instruction $p_t$\\
   {\tiny what is true, in model language}};
\node[devrow, anchor=north, minimum width=54mm, fill=contgreen!55] at (64.5,40.5) (r4)
  {\textbf{4.} \textbf{Continuity latch}: anchor $f_t$\\
   {\tiny what the world looks like now}};
\draw[flow] (r1.south) -- (r2.north);
\draw[flow] (r2.south) -- (r3.north);
\draw[flow] (r3.south) -- (r4.north);
\node[font=\tiny\bfseries, text=harnessbluedark] at (64.5,24.2) {\sysname{}: deterministic code, no learned weights};

% intermediate-result slots (reserved for real renders)
\draw[slot, draw=spatialorangedark, fill=spatialorange!12] (100,56) rectangle (124,69);
\begin{scope}[shift={(110,62.6)}, scale=0.58]\whitescene{0}{0}\end{scope}
\begin{scope}[shift={(119.5,58.4)}]
  \draw[black!60, fill=black!30, line width=0.4] (0,0.4) -- (2.0,1.3) -- (2.0,2.1) -- (0,1.2) -- cycle;
  \draw[black!60, line width=0.5] (0.4,0.4) -- (0.4,-1.0);
  \draw[black!60, line width=0.5] (1.6,0.9) -- (1.6,-0.6);
\end{scope}
\node[font=\tiny, text=spatialorangedark] at (112,58.1) {previz clip $r_t$};
\draw[channel, draw=spatialorangedark] (r2.east) -- (100,62.5);
\draw[slot, draw=harnessbluedark, fill=harnessblue!12] (100,40) rectangle (124,53);
\docglyph{112}{48.4};
\node[font=\tiny, text=harnessbluedark] at (112,42.1) {instruction $p_t$};
\draw[channel, draw=harnessbluedark] (r3.east) -- (100,46.5);
\draw[slot, draw=contgreendark, fill=contgreen!14] (100,24) rectangle (124,37);
\node[font=\tiny\itshape, text=contgreendark!70, align=center] at (112,30.5)
  {anchor $f_t$\\[1pt]{\tiny frame slot}};
\draw[channel, draw=contgreendark] (r4.east) -- (100,30.5);

% video model
\node[draw=modelgreydark, fill=modelgrey, rounded corners=1.5pt, thick, align=center,
      minimum width=25mm, minimum height=16mm] at (140,48) (vm)
  {\textbf{Video world model}\\ $V_\theta$\\ {\tiny weight-frozen, pluggable}};
\draw[channel, draw=spatialorangedark] (124,62.5) -- ($(vm.north west)+(1.5mm,-1mm)$);
\draw[channel, draw=harnessbluedark] (124,46.5) -- (vm.west);
\draw[channel, draw=contgreendark] (124,30.5) -- ($(vm.south west)+(1.5mm,1mm)$);
\fill[spatialorangedark] ($(vm.north west)+(1.5mm,-1mm)$) circle (0.65);
\fill[harnessbluedark] (vm.west) circle (0.65);
\fill[contgreendark] ($(vm.south west)+(1.5mm,1mm)$) circle (0.65);

% clip slot + verifier
\draw[slot, draw=black!50, fill=black!4] (160,41) rectangle (182,55);
\node[font=\tiny\itshape, text=black!45, align=center] at (171,48)
  {clip $v_t$\\[1pt]{\tiny video slot}};
\draw[arr] (vm.east) -- (160,48);
\node[draw=black!55, dashed, rounded corners=1.5pt, thick, fill=white, align=center, inner sep=2pt,
      minimum width=22mm] at (171,26) (verif) {\textbf{Verifier} $\varphi$ {\tiny (eval only)}\\ {\tiny closed-form twin QA}};
\draw[feedback] (171,41) -- (verif.north);

% feedback: last settled frame -> latch (next turn)
\draw[feedback, line width=0.7pt] (182,17) -| (17,22)
  node[pos=0.30, above, font=\tiny, black!55]{last settled frame anchors the next turn (display only)};
\draw[feedback, line width=0.7pt] (182,48) -- (182,17);

% ================= discipline strip =================
\draw[harnessbluedark, rounded corners=2pt, thick, fill=harnessblue!25] (2,2) rectangle (188,10.5);
\node[font=\tiny, align=center, text=black!80] at (95,6.25)
  {\textbf{\textcolor{harnessbluedark}{Settle before render:}} no pixel is generated until $\tau$ resolves the turn\\[1pt]
   \textbf{\textcolor{harnessbluedark}{One-way dependency:}} every fact flows harness $\to$ model; $V_\theta$ never writes state};

\end{tikzpicture}}%
\caption{\textbf{The \sysname{}, staged.}
\textbf{(a)} Setup (once per world, per twin): a rule-program agent writes, validates, and
freezes the game's rule program; the user supplies the first frame; the ledger ($z_A \neq z_B$)
and the initial clay-model scene are initialized --- twins differ \emph{only} in ledger
contents. The inset shows the four primitives this defines: rules read the state and the
action and write the next state; goals end the episode. \textbf{(b)} Turn loop: the harness settles the turn in deterministic code, edits
the clay model, compiles the settled facts into the backend's native instruction, and
chains the anchor frame; the frozen model is consulted once through three one-way channels
--- previz reference $r_t$ (orange), text instruction $p_t$ (blue), anchor frame $f_t$
(green) --- and returns only pixels, whose last settled frame anchors the next turn. Dashed
slots reserve intermediate artifacts; the closed-form verifier $\varphi$ scores clips at
evaluation time only.}
\label{fig:framework}
\end{figure}


==> figures/fig_teaser.tex <==
% ------------------------------------------------------------------
% Figure 1 (teaser): counterfactual twin evaluation, chest-opening case.
% Absolute-coordinate layout (canvas ~208 x 100mm), \resizebox to \textwidth.
% Image regions are EMPTY SLOTS (\figslot): photographic frames and ending
% clips are generated separately (see figures/FIGURE_PROMPTS.md) and drop in
% via \includegraphics at the slot's exact position and size.
% ------------------------------------------------------------------
\begin{figure}[t]
\centering
\resizebox{0.75\textwidth}{!}{%
\begin{tikzpicture}[
  font=\scriptsize, x=1mm, y=1mm,
  panel/.style={draw=black!55, rounded corners=2pt, thick},
  hlbl/.style={font=\tiny\bfseries, align=center},
  arr/.style={-{Latex[length=2.2mm]}, line width=0.8pt},
  rail/.style={-{Latex[length=2.2mm]}, line width=0.7pt, contgreendark},
]

% ===== framed slot with twin badge ================================
% #1=x  #2=y (south-west of a 26 x 14.6 slot)  #3=badge letter or '-'
% #4=badge color   #5=slot label
\newcommand{\twinslot}[5]{%
  \figslot{#1}{#2}{26}{14.6}{#5}
  \ifx&#3&\else
    \draw[black!50, fill=white, line width=0.6] ({#1+3.0},{#2+11.6}) circle (1.7);
    \node[font=\tiny\bfseries, #4] at ({#1+3.0},{#2+11.55}) {#3};
  \fi
}

% ===== status chip macro =========================================
% #1=x #2=y #3=label(A/B) #4=chip color #5=value(false/true) #6=rule consequence
\newcommand{\statechip}[6]{%
  \draw[black!45, rounded corners=1.2pt, fill=white, line width=0.5]
    (#1,#2) rectangle ({#1+58},{#2+4.6});
  \draw[#4, fill=#4, line width=0.6] ({#1+2.6},{#2+2.3}) circle (1.45);
  \node[font=\tiny\bfseries, white] at ({#1+2.6},{#2+2.25}) {#3};
  \node[font=\tiny, black!80, anchor=west] at ({#1+5.4},{#2+2.3})
    {\texttt{has\_key}~$=$~#5};
  \node[font=\tiny, black!65, anchor=east] at ({#1+56},{#2+2.3}) {#6};
}

% ===== top row: what each side receives ==========================
\draw[panel, fill=black!4] (2,72) rectangle (62,98);
\node[hlbl, anchor=north] at (32,97.2) {Shared surface --- identical frame \& request};
\twinslot{8}{76.6}{}{black!0}{first frame $I_0$\\[1pt]{\tiny photo: chest, character}}
\node[font=\tiny, black!70, align=center] at (46,83.5) {identical action:\\[2pt] ``open the chest''};

\draw[panel, fill=harnessblue!18, draw=harnessbluedark] (68,72) rectangle (134,98);
\node[hlbl, text=harnessbluedark, anchor=north] at (101,97.2)
  {Hidden state $S_{\mathrm{sem}}$ \textnormal{\tiny (ledger: invisible to $V_\theta$)}};
\statechip{72}{88.6}{A}{spatialorangedark}{false}{open must fail}
\statechip{72}{82.6}{B}{harnessbluedark}{true}{open must succeed}
\node[font=\tiny, black!60, anchor=north] at (101,81.4)
  {neither value can be read from the frame --- only the rules decide};

% ===== raw lane ==================================================
\draw[panel, fill=failred!8, draw=failred] (2,38) rectangle (160,68);
\node[hlbl, text=failred, anchor=north west] at (5,67.2)
  {Raw video world model --- state implicit in pixels and prose};
\twinslot{8}{43.0}{A}{spatialorangedark}{ending clip, twin A\\[1pt]{\tiny chest opens, gold}}
\twinslot{38}{43.0}{B}{harnessbluedark}{ending clip, twin B\\[1pt]{\tiny chest opens, gold (same)}}
\draw[failred, densely dashed, line width=0.6, -{Latex[length=1.6mm]}]
  (21,58.4) -- (21,60.8) -- (51,60.8) -- (51,58.4);
\node[font=\tiny\itshape, text=black!55] at (36,62.3) {identical pixels in, identical pixels out};
\node[font=\tiny, black!60, anchor=north] at (21,41.6) {ending: chest opens};
\node[font=\tiny, black!60, anchor=north] at (51,41.6) {ending: chest opens};
\node[hlbl, align=left, anchor=west, text=black!75] at (68,54)
  {the chest opens in both twins --- no key required\\[2pt]
   \textcolor{failred}{\textbf{twin collapse} (\textsc{CopyPaste}: 34\% of twin pairs)}\\[2pt]
   {\tiny the model's prior wins over the stated facts}};

% ===== harness lane ==============================================
\draw[panel, fill=contgreen!10, draw=contgreendark] (2,4) rectangle (160,34);
\node[hlbl, text=contgreendark, anchor=north west] at (5,33.2)
  {\sysname{} --- state explicit: rules, ledger, clay model};
\twinslot{8}{9.0}{A}{spatialorangedark}{ending clip, twin A\\[1pt]{\tiny lid locked, hands strain}}
\twinslot{38}{9.0}{B}{harnessbluedark}{ending clip, twin B\\[1pt]{\tiny lid open, gold, key raised}}
\node[font=\tiny, black!60, anchor=north] at (21,7.6) {ending A: lid will not budge};
\node[font=\tiny, black!60, anchor=north] at (51,7.6) {ending B: gold, key in hand};
\node[hlbl, align=left, anchor=west, text=black!75] at (68,20)
  {outcomes settle in code \emph{before} rendering --- twins diverge as the rules require\\[2pt]
   \textcolor{contgreendark}{\textbf{visibly different, rule-consistent endings} (\textsc{PairFollow}: 88\%)}\\[2pt]
   {\tiny twin A: hands strain on a locked lid \quad twin B: lid open, key raised}};

% ===== arrows ====================================================
% raw model consumes only the shared surface
\draw[arr, failred] (32,72) -- (32,68.6);
\node[font=\tiny\itshape, text=black!60, anchor=west] at (34,70.3) {raw model sees only the surface};
% rails on the right: harness consumes surface AND hidden state
\draw[rail] (62,94) -- (166,94) -- (166,22.5) -- (160.6,22.5);
\draw[rail] (134,90) -- (172.5,90) -- (172.5,15.5) -- (160.6,15.5);
\node[font=\tiny\itshape, text=contgreendark, rotate=90, anchor=south] at (164.6,52) {frame + action};
\node[font=\tiny\itshape, text=contgreendark, rotate=90, anchor=south] at (171.2,52) {+ hidden state};

\end{tikzpicture}}
\caption{\textbf{Counterfactual twins expose the missing state in video world models.}
Both twins share an identical first frame and an identical player action; they differ only in
hidden state that a frozen model cannot see --- here, \texttt{has\_key}. A raw video world
model receives only the shared surface and renders the same clip twice: the chest opens in
both twins, the model's prior overriding the stated facts (middle lane). The \sysname{}
additionally reads the hidden-state ledger, settles the outcome in deterministic code
\emph{before} rendering, and controls the same frozen model through a text channel (settled
facts) and a spatial channel (clay-model previz), so the twins diverge exactly as the rules
require (bottom lane).}
\label{fig:teaser}
\end{figure}

